Investigating the OPS intermediate representation to target GPUs in the Devito DSL

The Devito DSL is a code generation tool for the solution of partial differential equations using the finite difference method specifically aimed at seismic inversion problems. In this work we investigate the integration of OPS, an API to generate highly optimized code for applications running on structured meshes targeting various platforms, within Devito as a mean of bringing it to the GPU realm by providing an implementation of a OPS backend in Devito, obtaining considerable speed ups compared to the core Devito backend.

==> plan/plan.tex <==
\chapter{Plan}
Work for this project will be carried out following the software engineering methodologies currently used in the development of Devito. This will enable the results of this work to be part of future Devito releases and not be confined to an experimental branch, only created for the purposes of this project.

The project will be considered completed when common inversion problems can be solved in Devito using the OPS backend running on GPUs with acceptable performance. 

\begin{itemize}[listparindent=\parindent]
    \item Incrementally develop basic features and document them in the report
    \item \textbf{Milestone}: simple kernels compiled via OPS and run on CPUs (exp. Feb)
    \item Evaluation of the complexity that will arise when trying to run on GPUs
    \item Produce an analysis of the most important issues when working with GPUs in Devito 
    \item \textbf{Milestone}: simple kernels compile via OPS and run on GPUs (exp. Feb)
    \item Develop missing features required to compile and run basic seismic equations
    \item \textbf{Milestone}: compile and run Acoustic Wave Equation on CPUs (exp. Mar)
    \item Produce performance graphs and evaluate against Devito default back-end
    \item \textbf{Milestone}: compile and run Acoustic Wave Equation on GPUs (exp. Mar)
    \item Produce performance graphs and evaluate against Devito default back-end
    \item If on track, focus on more complex inversion problems
    \item Report writing
\end{itemize}
